Visual Question Answering: A Survey on Techniques and Common Trends in Recent Literature

Visual Question Answering (VQA) is an emerging area of interest for researches, being a recent problem in natural language processing and image prediction. In this area, an algorithm needs to answer questions about certain images. As of the writing of this survey, 25 recent studies were analyzed. Besides, 6 datasets were analyzed and provided their link to download. In this work, several recent pieces of research in this area were investigated and a deeper analysis and comparison among them were provided, including results, the state-of-the-art, common errors, and possible points of improvement for future researchers.

==> sections/refs.tex <==
@inproceedings{PaLI,
	
	title	= {PaLI: A Jointly-Scaled Multilingual Language-Image Model},
	
	author	= {Xi Chen and Xiao Wang and Soravit Changpinyo and AJ Piergiovanni and Piotr Padlewski and Daniel Salz and Sebastian Alexander Goodman and Adam Grycner and Basil Mustafa and Lucas Beyer and Alexander Kolesnikov and Joan Puigcerver and Nan Ding and Keran Rong and Hassan Akbari and Gaurav Mishra and Linting Xue and Ashish Thapliyal and James Bradbury and Weicheng Kuo and Mojtaba Seyedhosseini and Chao Jia and Burcu Karagol Ayan and Carlos Riquelme and Andreas Steiner and Anelia Angelova and Xiaohua Zhai and Neil Houlsby and Radu Soricut},
	year	= {2023},
	URL	= {https://arxiv.org/abs/2209.06794}
}

@inproceedings{MUSTVQA,
	author = {Vivoli, Emanuele and Biten, Ali Furkan and Mafla, Andres and Karatzas, Dimosthenis and Gomez, Lluis},
	title = {MUST-VQA: MUltilingual Scene-Text VQA},
	year = {2023},
	isbn = {978-3-031-25068-2},
	publisher = {Springer-Verlag},
	address = {Berlin, Heidelberg},
	url = {https://doi.org/10.1007/978-3-031-25069-9_23},
	doi = {10.1007/978-3-031-25069-9_23},
	booktitle = {Computer Vision – ECCV 2022 Workshops: Tel Aviv, Israel, October 23–27, 2022, Proceedings, Part IV},
	pages = {345–358},
	numpages = {14},
	location = {Tel Aviv, Israel}
}

@INPROCEEDINGS {kervadec2021transferable,
	author = {C. Kervadec and T. Jaunet and G. Antipov and M. Baccouche and R. Vuillemot and C. Wolf},
	booktitle = {2021 IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR)},
	title = {How Transferable are Reasoning Patterns in VQA?},
	year = {2021},
	volume = {},
	issn = {},
	pages = {4205-4214},
	doi = {10.1109/CVPR46437.2021.00419},
	url = {https://doi.ieeecomputersociety.org/10.1109/CVPR46437.2021.00419},
	publisher = {IEEE Computer Society},
	address = {Los Alamitos, CA, USA},
	month = {jun}
}
@inproceedings{lxmert,
	title = "{LXMERT}: Learning Cross-Modality Encoder Representations from Transformers",
	author = "Tan, Hao  and
	Bansal, Mohit",
	booktitle = "Proceedings of the 2019 Conference on Empirical Methods in Natural Language Processing and the 9th International Joint Conference on Natural Language Processing (EMNLP-IJCNLP)",
	month = nov,
	year = "2019",
	address = "Hong Kong, China",
	publisher = "Association for Computational Linguistics",
	url = "https://aclanthology.org/D19-1514",
	doi = "10.18653/v1/D19-1514",
	pages = "5100--5111",
}
@article{hopfield,
  title={Hopfield Networks is All You Need},
  author={Ramsauer, Hubert and Sch{\"a}fl, Bernhard and Lehner, Johannes and Seidl, Philipp and Widrich, Michael and Adler, Thomas and Gruber, Lukas and Holzleitner, Markus and Pavlovi{\'c}, Milena and Sandve, Geir Kjetil and others},
  journal={arXiv preprint arXiv:2008.02217},
  doi={https://doi.org/10.48550/arXiv.2008.02217},
  year={2020}
}
@InProceedings{STVQA_original,
	author = {Biten, Ali Furkan and Tito, Ruben and Mafla, Andres and Gomez, Lluis and Rusinol, Marcal and Valveny, Ernest and Jawahar, C.V. and Karatzas, Dimosthenis},
	title = {Scene Text Visual Question Answering},
	booktitle = {Proceedings of the IEEE/CVF International Conference on Computer Vision (ICCV)},
	month = {October},
	year = {2019}
}
@inproceedings{Faster_RCNN,
	author = {Ren, Shaoqing and He, Kaiming and Girshick, Ross and Sun, Jian},
	booktitle = {Advances in Neural Information Processing Systems},
	editor = {C. Cortes and N. Lawrence and D. Lee and M. Sugiyama and R. Garnett},
	pages = {},
	publisher = {Curran Associates, Inc.},
	title = {Faster R-CNN: Towards Real-Time Object Detection with Region Proposal Networks},
	url = {https://proceedings.neurips.cc/paper_files/paper/2015/file/14bfa6bb14875e45bba028a21ed38046-Paper.pdf},
	volume = {28},
	year = {2015}
}
@article{ImageNet,
	Author = {Olga Russakovsky and Jia Deng and Hao Su and Jonathan Krause and Sanjeev Satheesh and Sean Ma and Zhiheng Huang and Andrej Karpathy and Aditya Khosla and Michael Bernstein and Alexander C. Berg and Li Fei-Fei},
	Title = {{ImageNet Large Scale Visual Recognition Challenge}},
	Year = {2015},
	journal   = {International Journal of Computer Vision (IJCV)},
	doi = {10.1007/s11263-015-0816-y},
	volume={115},
	number={3},
	pages={211-252}
}
@article{Visual_Genome,
	author = {Krishna, Ranjay and Zhu, Yuke and Groth, Oliver and Johnson, Justin and Hata, Kenji and Kravitz, Joshua and Chen, Stephanie and Kalantidis, Yannis and Li, Li-Jia and Shamma, David A. and Bernstein, Michael S. and Fei-Fei, Li},
	title = {Visual Genome: Connecting Language and Vision Using Crowdsourced Dense Image Annotations},
	year = {2017},
	issue_date = {May       2017},
	publisher = {Kluwer Academic Publishers},
	address = {USA},
	volume = {123},
	number = {1},
	issn = {0920-5691},
	url = {https://doi.org/10.1007/s11263-016-0981-7},
	doi = {10.1007/s11263-016-0981-7},
	abstract = {Despite progress in perceptual tasks such as image classification, computers still perform poorly on cognitive tasks such as image description and question answering. Cognition is core to tasks that involve not just recognizing, but reasoning about our visual world. However, models used to tackle the rich content in images for cognitive tasks are still being trained using the same datasets designed for perceptual tasks. To achieve success at cognitive tasks, models need to understand the interactions and relationships between objects in an image. When asked "What vehicle is the person riding?", computers will need to identify the objects in an image as well as the relationships riding(man, carriage) and pulling(horse, carriage) to answer correctly that "the person is riding a horse-drawn carriage." In this paper, we present the Visual Genome dataset to enable the modeling of such relationships. We collect dense annotations of objects, attributes, and relationships within each image to learn these models. Specifically, our dataset contains over 108K images where each image has an average of $$35$$35 objects, $$26$$26 attributes, and $$21$$21 pairwise relationships between objects. We canonicalize the objects, attributes, relationships, and noun phrases in region descriptions and questions answer pairs to WordNet synsets. Together, these annotations represent the densest and largest dataset of image descriptions, objects, attributes, relationships, and question answer pairs.},
	journal = {Int. J. Comput. Vision},
	month = {may},
	pages = {32–73},
	numpages = {42},
	keywords = {Objects, Attributes, Language, Scene graph, Crowdsourcing, Dataset, Question answering, Knowledge, Image, Relationships, Computer vision}
}
@InProceedings{BPEmb,
	author = {Benjamin Heinzerling and Michael Strube},
	title = "{BPEmb: Tokenization-free Pre-trained Subword Embeddings in 275 Languages}",
	booktitle = {Proceedings of the Eleventh International Conference on Language Resources and Evaluation (LREC 2018)},
	year = {2018},
	month = {May 7-12, 2018},
	address = {Miyazaki, Japan},
	editor = {Nicoletta Calzolari (Conference chair) and Khalid Choukri and Christopher Cieri and Thierry Declerck and Sara Goggi and Koiti Hasida and Hitoshi Isahara and Bente Maegaard and Joseph Mariani and Hélène Mazo and Asuncion Moreno and Jan Odijk and Stelios Piperidis and Takenobu Tokunaga},
	publisher = {European Language Resources Association (ELRA)},
	isbn = {979-10-95546-00-9},
	language = {english}
}
@article{T5,
	author = {Raffel, Colin and Shazeer, Noam and Roberts, Adam and Lee, Katherine and Narang, Sharan and Matena, Michael and Zhou, Yanqi and Li, Wei and Liu, Peter J.},
	title = {Exploring the Limits of Transfer Learning with a Unified Text-to-Text Transformer},
	year = {2020},
	issue_date = {January 2020},
	publisher = {JMLR.org},
	volume = {21},
	number = {1},
	issn = {1532-4435},
	abstract = {Transfer learning, where a model is first pre-trained on a data-rich task before being fine-tuned on a downstream task, has emerged as a powerful technique in natural language processing (NLP). The effectiveness of transfer learning has given rise to a diversity of approaches, methodology, and practice. In this paper, we explore the landscape of transfer learning techniques for NLP by introducing a unified framework that converts all text-based language problems into a text-to-text format. Our systematic study compares pretraining objectives, architectures, unlabeled data sets, transfer approaches, and other factors on dozens of language understanding tasks. By combining the insights from our exploration with scale and our new "Colossal Clean Crawled Corpus", we achieve state-of-the-art results on many benchmarks covering summarization, question answering, text classification, and more. To facilitate future work on transfer learning for NLP, we release our data set, pre-trained models, and code.},
	journal = {J. Mach. Learn. Res.},
	month = {jan},
	articleno = {140},
	numpages = {67},
	keywords = {attention based models, multi-task learning, deep learning, natural language processing, transfer learning}
}
@inproceedings{mt5,
	title = "m{T}5: A Massively Multilingual Pre-trained Text-to-Text Transformer",
	author = "Xue, Linting  and
	Constant, Noah  and
	Roberts, Adam  and
	Kale, Mihir  and
	Al-Rfou, Rami  and
	Siddhant, Aditya  and
	Barua, Aditya  and
	Raffel, Colin",
	booktitle = "Proceedings of the 2021 Conference of the North American Chapter of the Association for Computational Linguistics: Human Language Technologies",
	month = jun,
	year = "2021",
	address = "Online",
	publisher = "Association for Computational Linguistics",
	url = "https://aclanthology.org/2021.naacl-main.41",
	doi = "10.18653/v1/2021.naacl-main.41",
	pages = "483--498",
	abstract = "The recent {``}Text-to-Text Transfer Transformer{''} (T5) leveraged a unified text-to-text format and scale to attain state-of-the-art results on a wide variety of English-language NLP tasks. In this paper, we introduce mT5, a multilingual variant of T5 that was pre-trained on a new Common Crawl-based dataset covering 101 languages. We detail the design and modified training of mT5 and demonstrate its state-of-the-art performance on many multilingual benchmarks. We also describe a simple technique to prevent {``}accidental translation{''} in the zero-shot setting, where a generative model chooses to (partially) translate its prediction into the wrong language. All of the code and model checkpoints used in this work are publicly available.",
}
@INPROCEEDINGS{LaTr,
	author={Biten, Ali Furkan and Litman, Ron and Xie, Yusheng and Appalaraju, Srikar and Manmatha, R.},
	booktitle={2022 IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR)}, 
	title={LaTr: Layout-Aware Transformer for Scene-Text VQA}, 
	year={2022},
	volume={},
	number={},
	pages={16527-16537},
	doi={10.1109/CVPR52688.2022.01605},
	ISSN={2575-7075},
	month={June},}
@article{FastText,
	author = {Bojanowski, Piotr and Grave, Edouard and Joulin, Armand and Mikolov, Tomas},
	title = "{Enriching Word Vectors with Subword Information}",
	journal = {Transactions of the Association for Computational Linguistics},
	volume = {5},
	pages = {135-146},
	year = {2017},
	month = {06},
	abstract = "{Continuous word representations, trained on large unlabeled corpora are useful
	for many natural language processing tasks. Popular models that learn such
	representations ignore the morphology of words, by assigning a distinct vector
	to each word. This is a limitation, especially for languages with large
	vocabularies and many rare words. In this paper, we propose a new approach based
	on the skipgram model, where each word is represented as a bag of character n-grams. A vector representation is associated
	to each character n-gram; words being represented
	as the sum of these representations. Our method is fast, allowing to train
	models on large corpora quickly and allows us to compute word representations
	for words that did not appear in the training data. We evaluate our word
	representations on nine different languages, both on word similarity and analogy
	tasks. By comparing to recently proposed morphological word representations, we
	show that our vectors achieve state-of-the-art performance on these tasks.}",
	issn = {2307-387X},
	doi = {10.1162/tacl_a_00051},
	url = {https://doi.org/10.1162/tacl\_a\_00051},
	eprint = {https://direct.mit.edu/tacl/article-pdf/doi/10.1162/tacl\_a\_00051/1567442/tacl\_a\_00051.pdf},
}
@ARTICLE{PHOC,
	author={Almazán, Jon and Gordo, Albert and Fornés, Alicia and Valveny, Ernest},
	journal={IEEE Transactions on Pattern Analysis and Machine Intelligence}, 
	title={Word Spotting and Recognition with Embedded Attributes}, 
	year={2014},
	volume={36},
	number={12},
	pages={2552-2566},
	doi={10.1109/TPAMI.2014.2339814}}
@INPROCEEDINGS{TextVQA,
	author={Singh, Amanpreet and Natarajan, Vivek and Shah, Meet and Jiang, Yu and Chen, Xinlei and Batra, Dhruv and Parikh, Devi and Rohrbach, Marcus},
	booktitle={2019 IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR)}, 
	title={Towards VQA Models That Can Read}, 
	year={2019},
	volume={},
	number={},
	pages={8309-8318},
	doi={10.1109/CVPR.2019.00851}}
@inproceedings{Rosetta_OCR,
	author = {Borisyuk, Fedor and Gordo, Albert and Sivakumar, Viswanath},
	title = {Rosetta: Large Scale System for Text Detection and Recognition in Images},
	year = {2018},
	isbn = {9781450355520},
	publisher = {Association for Computing Machinery},
	address = {New York, NY, USA},
	url = {https://doi.org/10.1145/3219819.3219861},
	doi = {10.1145/3219819.3219861},
	abstract = {In this paper we present a deployed, scalable optical character recognition (OCR) system, which we call Rosetta , designed to process images uploaded daily at Facebook scale. Sharing of image content has become one of the primary ways to communicate information among internet users within social networks such as Facebook, and the understanding of such media, including its textual information, is of paramount importance to facilitate search and recommendation applications. We present modeling techniques for efficient detection and recognition of text in images and describe Rosetta 's system architecture. We perform extensive evaluation of presented technologies, explain useful practical approaches to build an OCR system at scale, and provide insightful intuitions as to why and how certain components work based on the lessons learnt during the development and deployment of the system.},
	booktitle = {Proceedings of the 24th ACM SIGKDD International Conference on Knowledge Discovery and Data Mining},
	pages = {71–79},
	numpages = {9},
	keywords = {text recognition, text detection, optical character recognition},
	location = {London, United Kingdom},
	series = {KDD '18}
}
@article{Adam_original,
	title={Adam: A Method for Stochastic Optimization},
	author={Diederik P. Kingma and Jimmy Ba},
	journal={CoRR},
	year={2014},
	volume={abs/1412.6980}
}
@inproceedings{AdamW,
	author    = {Ilya Loshchilov and
	Frank Hutter},
	title     = {Decoupled Weight Decay Regularization},
	booktitle = {7th International Conference on Learning Representations, {ICLR} 2019,
	New Orleans, LA, USA, May 6-9, 2019},
	publisher = {OpenReview.net},
	year      = {2019},
	url       = {https://openreview.net/forum?id=Bkg6RiCqY7},
	timestamp = {Thu, 25 Jul 2019 14:26:04 +0200},
	biburl    = {https://dblp.org/rec/conf/iclr/LoshchilovH19.bib},
	bibsource = {dblp computer science bibliography, https://dblp.org}
}
@inproceedings{Amazon-OCR,
	author = {Ughetta, William and Kernighan, Brian},
	year = {2020},
	month = {09},
	pages = {1-4},
	title = {The Old Bailey and OCR: Benchmarking AWS, Azure, and GCP with 180,000 Page Images},
	doi = {10.1145/3395027.3419595}
}
@inproceedings{
	ViT,
	title={An Image is Worth 16x16 Words: Transformers for Image Recognition at Scale},
	author={Alexey Dosovitskiy and Lucas Beyer and Alexander Kolesnikov and Dirk Weissenborn and Xiaohua Zhai and Thomas Unterthiner and Mostafa Dehghani and Matthias Minderer and Georg Heigold and Sylvain Gelly and Jakob Uszkoreit and Neil Houlsby},
	booktitle={International Conference on Learning Representations},
	year={2021},
	url={https://openreview.net/forum?id=YicbFdNTTy}
}
@article{Liu2022,
	doi = {10.1145/3498340},
	url = {https://doi.org/10.1145/3498340},
	year = {2022},
	month = nov,
	publisher = {Association for Computing Machinery ({ACM})},
	volume = {18},
	number = {4},
	pages = {1--18},
	author = {Yibing Liu and Yangyang Guo and Jianhua Yin and Xuemeng Song and Weifeng Liu and Liqiang Nie and Min Zhang},
	title = {Answer Questions with Right Image Regions: A Visual Attention Regularization Approach},
	journal = {{ACM} Transactions on Multimedia Computing,  Communications,  and Applications}
}
@InProceedings{survey_vqa,
	author="Srivastava, Yash
	and Murali, Vaishnav
	and Dubey, Shiv Ram
	and Mukherjee, Snehasis",
	editor="Singh, Satish Kumar
	and Roy, Partha
	and Raman, Balasubramanian
	and Nagabhushan, P.",
	title="Visual Question Answering Using Deep Learning: A Survey and Performance Analysis",
	booktitle="Computer Vision and Image Processing",
	year="2021",
	publisher="Springer Singapore",
	address="Singapore",
	pages="75--86",
	isbn="978-981-16-1092-9"
}

@inproceedings{gru-original,
	title = "Learning Phrase Representations using {RNN} Encoder{--}Decoder for Statistical Machine Translation",
	author = {Cho, Kyunghyun  and
	van Merri{\"e}nboer, Bart  and
	Gulcehre, Caglar  and
	Bahdanau, Dzmitry  and
	Bougares, Fethi  and
	Schwenk, Holger  and
	Bengio, Yoshua},
	booktitle = "Proceedings of the 2014 Conference on Empirical Methods in Natural Language Processing ({EMNLP})",
	month = oct,
	year = "2014",
	address = "Doha, Qatar",
	publisher = "Association for Computational Linguistics",
	url = "https://aclanthology.org/D14-1179",
	doi = "10.3115/v1/D14-1179",
	pages = "1724--1734",
}

@INPROCEEDINGS{teneynet,
	author={Teney, Damien and Anderson, Peter and He, Xiaodong and Hengel, Anton van den},
	booktitle={2018 IEEE/CVF Conference on Computer Vision and Pattern Recognition}, 
	title={Tips and Tricks for Visual Question Answering: Learnings from the 2017 Challenge}, 
	year={2018},
	volume={},
	number={},
	pages={4223-4232},
	doi={10.1109/CVPR.2018.00444},
	ISSN={2575-7075},
	month={June},}



@inproceedings{VQAoriginal,
	author = {Stanislaw Antol and Aishwarya Agrawal and Jiasen Lu and Margaret Mitchell and Dhruv Batra and C. Lawrence Zitnick and Devi Parikh},
	title = {{VQA}: {V}isual {Q}uestion {A}nswering},
	booktitle = {International Conference on Computer Vision (ICCV)},
	year = {2015},
}

@article{robertson2004understanding,
	title = {Understanding inverse document frequency: on theoretical arguments for IDF},
	author = {Robertson, Stephen},
	journal = {Journal of documentation},
	year = {2004},
	publisher = {Emerald Group Publishing Limited}
}
@inproceedings{bert-original,
	title = "{BERT}: Pre-training of Deep Bidirectional Transformers for Language Understanding",
	author = "Devlin, Jacob  and
	Chang, Ming-Wei  and
	Lee, Kenton  and
	Toutanova, Kristina",
	booktitle = "Proceedings of the 2019 Conference of the North {A}merican Chapter of the Association for Computational Linguistics: Human Language Technologies, Volume 1 (Long and Short Papers)",
	month = jun,
	year = "2019",
	address = "Minneapolis, Minnesota",
	publisher = "Association for Computational Linguistics",
	url = "https://aclanthology.org/N19-1423",
	doi = "10.18653/v1/N19-1423",
	pages = "4171--4186",
	abstract = "We introduce a new language representation model called BERT, which stands for Bidirectional Encoder Representations from Transformers. Unlike recent language representation models (Peters et al., 2018a; Radford et al., 2018), BERT is designed to pre-train deep bidirectional representations from unlabeled text by jointly conditioning on both left and right context in all layers. As a result, the pre-trained BERT model can be fine-tuned with just one additional output layer to create state-of-the-art models for a wide range of tasks, such as question answering and language inference, without substantial task-specific architecture modifications. BERT is conceptually simple and empirically powerful. It obtains new state-of-the-art results on eleven natural language processing tasks, including pushing the GLUE score to 80.5 (7.7 point absolute improvement), MultiNLI accuracy to 86.7{\%} (4.6{\%} absolute improvement), SQuAD v1.1 question answering Test F1 to 93.2 (1.5 point absolute improvement) and SQuAD v2.0 Test F1 to 83.1 (5.1 point absolute improvement).",
}
@inproceedings{sbd-trans-1,
	title     = {Omnidirectional Scene Text Detection with Sequential-free Box Discretization},
	author    = {Liu, Yuliang and Zhang, Sheng and Jin, Lianwen and Xie, Lele and Wu, Yaqiang and Wang, Zhepeng},
	booktitle = {Proceedings of the Twenty-Eighth International Joint Conference on
	Artificial Intelligence, {IJCAI-19}},
	publisher = {International Joint Conferences on Artificial Intelligence Organization},
	pages     = {3052--3058},
	year      = {2019},
	month     = {7},
	doi       = {10.24963/ijcai.2019/423},
	url       = {https://doi.org/10.24963/ijcai.2019/423},
}
@article{sbd-trans-2,
	title = {A holistic representation guided attention network for scene text recognition},
	journal = {Neurocomputing},
	volume = {414},
	pages = {67-75},
	year = {2020},
	issn = {0925-2312},
	doi = {https://doi.org/10.1016/j.neucom.2020.07.010},
	url = {https://www.sciencedirect.com/science/article/pii/S0925231220311176},
	author = {Lu Yang and Peng Wang and Hui Li and Zhen Li and Yanning Zhang},
	keywords = {Holistic Representation, Convolutional-Attention, Transformer, Scene Text Recognition},
}
@inproceedings{vedantam2015cider,
	title={Cider: Consensus-based image description evaluation},
	author={Vedantam, Ramakrishna and Lawrence Zitnick, C and Parikh, Devi},
	booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
	pages={4566--4575},
	year={2015}
}

@inproceedings{papineni2002bleu,
	title={Bleu: a method for automatic evaluation of machine translation},
	author={Papineni, Kishore and Roukos, Salim and Ward, Todd and Zhu, Wei-Jing},
	booktitle={Proceedings of the 40th annual meeting of the Association for Computational Linguistics},
	pages={311--318},
	year={2002}
}

@inproceedings{lin2003automatic,
	title={Automatic evaluation of summaries using n-gram co-occurrence statistics},
	author={Lin, Chin-Yew and Hovy, Eduard},
	booktitle={Proceedings of the 2003 human language technology conference of the North American chapter of the association for computational linguistics},
	pages={150--157},
	year={2003}
}

@inproceedings{rougepackage,
	title={Rouge: A package for automatic evaluation of summaries},
	author={Lin, Chin-Yew},
	booktitle={Text summarization branches out},
	pages={74--81},
	year={2004}
}
@inproceedings{vqa-hat,
	title = "Human Attention in Visual Question Answering: Do Humans and Deep Networks look at the same regions?",
	author = "Das, Abhishek  and
	Agrawal, Harsh  and
	Zitnick, Larry  and
	Parikh, Devi  and
	Batra, Dhruv",
	booktitle = "Proceedings of the 2016 Conference on Empirical Methods in Natural Language Processing",
	month = nov,
	year = "2016",
	address = "Austin, Texas",
	publisher = "Association for Computational Linguistics",
	url = "https://aclanthology.org/D16-1092",
	doi = "10.18653/v1/D16-1092",
	pages = "932--937",
}

@inproceedings{rougel,
	title={Automatic evaluation of machine translation quality using longest common subsequence and skip-bigram statistics},
	author={Lin, Chin-Yew and Och, Franz Josef},
	booktitle={Proceedings of the 42nd Annual Meeting of the Association for Computational Linguistics (ACL-04)},
	pages={605--612},
	year={2004}
}

@incollection{Salewski2022,
	doi = {10.1007/978-3-031-04083-2_5},
	url = {https://doi.org/10.1007/978-3-031-04083-2_5},
	year = {2022},
	publisher = {Springer International Publishing},
	pages = {69--88},
	author = {Leonard Salewski and A. Sophia Koepke and Hendrik P. A. Lensch and Zeynep Akata},
	title = {{CLEVR}-X: A Visual Reasoning Dataset for~Natural Language Explanations},
	booktitle = {{xxAI} - Beyond Explainable {AI}}
}
@INPROCEEDINGS{clevr,
	author={Johnson, Justin and Hariharan, Bharath and van der Maaten, Laurens and Fei-Fei, Li and Zitnick, C. Lawrence and Girshick, Ross},
	booktitle={2017 IEEE Conference on Computer Vision and Pattern Recognition (CVPR)}, 
	title={CLEVR: A Diagnostic Dataset for Compositional Language and Elementary Visual Reasoning}, 
	year={2017},
	volume={},
	number={},
	pages={1988-1997},
	doi={10.1109/CVPR.2017.215}
}

@InProceedings{okvqa,
	author = {Kenneth Marino and Mohammad Rastegari and Ali Farhadi and Roozbeh Mottaghi},
	title = {OK-VQA: A Visual Question Answering Benchmark Requiring External Knowledge},
	booktitle = {Conference on Computer Vision and Pattern Recognition (CVPR)},
	year = {2019},
}

@inproceedings{glove,
	author = {Jeffrey Pennington and Richard Socher and Christopher D. Manning},
	booktitle = {Empirical Methods in Natural Language Processing (EMNLP)},
	title = {GloVe: Global Vectors for Word Representation},
	year = {2014},
	pages = {1532--1543},
	url = {http://www.aclweb.org/anthology/D14-1162},
}
@inproceedings{Qu2021,
	doi = {10.1145/3404835.3462987},
	url = {https://doi.org/10.1145/3404835.3462987},
	year = {2021},
	month = jul,
	publisher = {{ACM}},
	author = {Chen Qu and Hamed Zamani and Liu Yang and W. Bruce Croft and Erik Learned-Miller},
	title = {Passage Retrieval for Outside-Knowledge Visual Question Answering},
	booktitle = {Proceedings of the 44th International {ACM} {SIGIR} Conference on Research and Development in Information Retrieval}
}



@inproceedings{Liang2021,
	doi = {10.1145/3404835.3462981},
	url = {https://doi.org/10.1145/3404835.3462981},
	year = {2021},
	month = jul,
	publisher = {{ACM}},
	author = {Zujie Liang and Haifeng Hu and Jiaying Zhu},
	title = {{LPF}: A Language-Prior Feedback Objective Function for De-biased Visual Question Answering},
	booktitle = {Proceedings of the 44th International {ACM} {SIGIR} Conference on Research and Development in Information Retrieval}
}
@inproceedings{cpigpaper,
	title = "A negative case analysis of visual grounding methods for {VQA}",
	author = "Shrestha, Robik  and
	Kafle, Kushal  and
	Kanan, Christopher",
	booktitle = "Proceedings of the 58th Annual Meeting of the Association for Computational Linguistics",
	month = jul,
	year = "2020",
	address = "Online",
	publisher = "Association for Computational Linguistics",
	url = "https://aclanthology.org/2020.acl-main.727",
	doi = "10.18653/v1/2020.acl-main.727",
	pages = "8172--8181",
}

@inproceedings{Han2021,
	doi = {10.1109/iccv48922.2021.00161},
	url = {https://doi.org/10.1109/iccv48922.2021.00161},
	year = {2021},
	month = oct,
	publisher = {{IEEE}},
	author = {Xinzhe Han and Shuhui Wang and Chi Su and Qingming Huang and Qi Tian},
	title = {Greedy Gradient Ensemble for Robust Visual Question Answering},
	booktitle = {2021 {IEEE}/{CVF} International Conference on Computer Vision ({ICCV})}
}



@inproceedings{https://doi.org/10.48550/arxiv.2111.02358,
	title={{VLM}o: Unified Vision-Language Pre-Training with Mixture-of-Modality-Experts},
	author={Hangbo Bao and Wenhui Wang and Li Dong and Qiang Liu and Owais Khan Mohammed and Kriti Aggarwal and Subhojit Som and Songhao Piao and Furu Wei},
	booktitle={Advances in Neural Information Processing Systems},
	editor={Alice H. Oh and Alekh Agarwal and Danielle Belgrave and Kyunghyun Cho},
	year={2022},
	url={https://openreview.net/forum?id=bydKs84JEyw}
}

@inproceedings{kafle2020answering,
	title={Answering questions about data visualizations using efficient bimodal fusion},
	author={Kafle, Kushal and Shrestha, Robik and Cohen, Scott and Price, Brian and Kanan, Christopher},
	booktitle={Proceedings of the IEEE/CVF Winter conference on applications of computer vision},
	pages={1498--1507},
	year={2020}
}

@inproceedings{nguyen2022coarse,
	title={Coarse-to-Fine Reasoning for Visual Question Answering},
	author={Nguyen, Binh X and Do, Tuong and Tran, Huy and Tjiputra, Erman and Tran, Quang D and Nguyen, Anh},
	booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
	pages={4558--4566},
	year={2022}
}

@inproceedings{hu2021question,
	title={Question-controlled Text-aware Image Captioning},
	author={Hu, Anwen and Chen, Shizhe and Jin, Qin},
	booktitle={Proceedings of the 29th ACM International Conference on Multimedia},
	pages={3097--3105},
	year={2021}
}

@misc{lin2022medical,
	title={Medical Visual Question Answering: A Survey}, 
	author={Zhihong Lin and Donghao Zhang and Qingyi Tac and Danli Shi and Gholamreza Haffari and Qi Wu and Mingguang He and Zongyuan Ge},
	year={2022},
	eprint={2111.10056},
	archivePrefix={arXiv},
	primaryClass={cs.CV}
}


@article{sharma2021survey,
	title = {A survey of methods, datasets and evaluation metrics for visual question answering},
	journal = {Image and Vision Computing},
	volume = {116},
	pages = {104327},
	year = {2021},
	issn = {0262-8856},
	doi = {https://doi.org/10.1016/j.imavis.2021.104327},
	url = {https://www.sciencedirect.com/science/article/pii/S0262885621002328},
	author = {Himanshu Sharma and Anand Singh Jalal},
	keywords = {Computer vision, Natural language processing, Deep neural networks, World knowledge, Attention},
	abstract = {Visual Question Answering (VQA) is a multi-disciplinary research problem that has captured the attention of both computer vision as well as natural language processing researchers. In Visual Question Answering, a system is given an image; a question in a natural language related to that image as an input, and the VQA system is required to give an answer in natural language as an output. A VQA algorithm may require common sense reasoning over the information contained in the image and world knowledge to produce the right answer. In this paper, we have discussed some of the core concepts used in VQA systems and present a comprehensive survey of efforts in the past to address this problem. Apart from traditional VQA models, we have also discussed visual question answering models that require reading texts present in images and evaluated on recently developed datasets like TextVQA, ST-VQA, and OCR-VQA. Apart from standard datasets discussed in previous surveys, we have also discussed some new datasets developed in 2019 and 2020 such as GQA, OK-VQA, TextVQA, ST-VQA, and OCR-VQA. The new evaluation metrics such as BLEU, MPT, METEOR, Average Normalized Levenshtein Similarity (ANLS), Validity, Plausibility, Distribution, Consistency, Grounding, F1-Score are explained together with the evaluation metrics discussed by previous surveys. We conclude our survey with a discussion on open issues in each phase of the VQA task and present some promising future directions.}
}


@article{manmadhan2020visual,
	title={Visual question answering: a state-of-the-art review},
	author={Manmadhan, Sruthy and Kovoor, Binsu C},
	journal={Artificial Intelligence Review},
	volume={53},
	pages={5705--5745},
	year={2020},
	publisher={Springer}
}


@article{patil2020visual,
	author = {Patil, Charulata and Patwardhan, Manasi},
	title = {Visual Question Generation: The State of the Art},
	year = {2020},
	issue_date = {May 2021},
	publisher = {Association for Computing Machinery},
	address = {New York, NY, USA},
	volume = {53},
	number = {3},
	issn = {0360-0300},
	url = {https://doi.org/10.1145/3383465},
	doi = {10.1145/3383465},
	abstract = {Visual question generation (VQG) is an interesting problem that has recently received attention. The task of VQG involves generating meaningful questions based on the input image. It is a multi-modal problem involving image understanding and natural language generation, especially using deep learning methods. VQG can be considered as complementary task of visual question answering. In this article, we review the current state of VQG in terms of methods to understand the problem, existing datasets to train the VQG model, evaluation metrics, and algorithms to handle the problem. Finally, we discuss the challenges that need to be conquered and the possible future directions for an effective VQG.},
	journal = {ACM Comput. Surv.},
	month = {may},
	articleno = {47},
	numpages = {22},
	keywords = {question generation, Image understanding}
}

@article{gong2021sysu,
	title={Sysu-hcp at vqa-med 2021: A data-centric model with efficient training methodology for medical visual question answering},
	author={Gong, Haifan and Huang, Ricong and Chen, Guanqi and Li, Guanbin},
	journal={Proceedings http://ceur-ws. org ISSN},
	volume={1613},
	pages={0073},
	year={2021}
}

@inbook{liu2021constrative,
	author = {Liu, Bo and Zhan, Li-Ming and Wu, Xiao-Ming},
	year = {2021},
	month = {09},
	pages = {210-220},
	title = {Contrastive Pre-training and Representation Distillation for Medical Visual Question Answering Based on Radiology Images},
	isbn = {978-3-030-87195-6},
	doi = {10.1007/978-3-030-87196-3_20}
}
@article{continual_learning_original,
	title={CHILD: A First Step Towards Continual Learning},
	author={Mark B. Ring},
	journal={Machine Learning},
	year={1997},
	volume={28},
	pages={77-104}
}
@inproceedings{wang2021mirtt,
	author = {Wang, Junjie and Ji, Yatai and Sun, Jiaqi and Yang, Yujiu and Sakai, Tetsuya},
	year = {2021},
	month = {01},
	pages = {2280-2292},
	title = {MIRTT: Learning Multimodal Interaction Representations from Trilinear Transformers for Visual Question Answering},
	doi = {10.18653/v1/2021.findings-emnlp.196}
}
@INPROCEEDINGS{yang2020learning,
	author={Yang, Chao and Feng, Su and Li, Dongsheng and Shen, Huawei and Wang, Guoqing and Jiang, Bin},
	booktitle={2021 IEEE International Conference on Multimedia and Expo (ICME)}, 
	title={Learning Content and Context with Language Bias for Visual Question Answering}, 
	year={2021},
	volume={},
	number={},
	pages={1-6},
	abstract={Visual Question Answering (VQA) is a challenging multi-modal task to answer questions about an image. Many works concentrate on how to reduce language bias which makes models answer questions ignoring visual content and language context. However, reducing language bias also weakens the ability of VQA models to learn context prior. To address this issue, we propose a novel learning strategy named CCB, which forces VQA models to answer questions relying on Content and Context with language Bias. Specifically, CCB establishes Content and Context branches on top of a base VQA model and forces them to focus on local key content and global effective context respectively. Moreover, a joint loss function is proposed to reduce the importance of biased samples and retain their beneficial influence on answering questions. Experiments show that CCB outperforms the state-of-the-art methods on VQA-CP v2.},
	keywords={},
	doi={10.1109/ICME51207.2021.9428098},
	ISSN={1945-788X},
	month={July},}

@misc{beit-sota,
	doi = {10.48550/ARXIV.2208.10442},
	
	url = {https://arxiv.org/abs/2208.10442},
	
	author = {Wang, Wenhui and Bao, Hangbo and Dong, Li and Bjorck, Johan and Peng, Zhiliang and Liu, Qiang and Aggarwal, Kriti and Mohammed, Owais Khan and Singhal, Saksham and Som, Subhojit and Wei, Furu},
	
	keywords = {Computer Vision and Pattern Recognition (cs.CV), Computation and Language (cs.CL), FOS: Computer and information sciences, FOS: Computer and information sciences},
	
	title = {Image as a Foreign Language: BEiT Pretraining for All Vision and Vision-Language Tasks},
	
	publisher = {arXiv},
	
	year = {2022},
	
	copyright = {arXiv.org perpetual, non-exclusive license}
}

@article{vqav2,
	author = {Goyal, Yash and Khot, Tejas and Agrawal, Aishwarya and Summers-Stay, Douglas and Batra, Dhruv and Parikh, Devi},
	title = {Making the V in VQA Matter: Elevating the Role of Image Understanding in Visual Question Answering},
	year = {2019},
	issue_date = {April     2019},
	publisher = {Kluwer Academic Publishers},
	address = {USA},
	volume = {127},
	number = {4},
	issn = {0920-5691},
	url = {https://doi.org/10.1007/s11263-018-1116-0},
	doi = {10.1007/s11263-018-1116-0},
	journal = {Int. J. Comput. Vision},
	month = {apr},
	pages = {398–414},
	numpages = {17},
	keywords = {Visual question answering, VQA, VQA challenge}
}
@inproceedings{vath2021beyond,
	title = "Beyond Accuracy: A Consolidated Tool for Visual Question Answering Benchmarking",
	author = {V{\"a}th, Dirk  and
	Tilli, Pascal  and
	Vu, Ngoc Thang},
	booktitle = "Proceedings of the 2021 Conference on Empirical Methods in Natural Language Processing: System Demonstrations",
	month = nov,
	year = "2021",
	address = "Online and Punta Cana, Dominican Republic",
	publisher = "Association for Computational Linguistics",
	url = "https://aclanthology.org/2021.emnlp-demo.14",
	doi = "10.18653/v1/2021.emnlp-demo.14",
	pages = "114--123",
}
@INPROCEEDINGS{farinhas2021multimodal,
	author = {A. Farinhas and A. T. Martins and P. Q. Aguiar},
	booktitle = {2021 IEEE/CVF International Conference on Computer Vision Workshops (ICCVW)},
	title = {Multimodal Continuous Visual Attention Mechanisms},
	year = {2021},
	volume = {},
	issn = {},
	pages = {1047-1056},
	doi = {10.1109/ICCVW54120.2021.00122},
	url = {https://doi.ieeecomputersociety.org/10.1109/ICCVW54120.2021.00122},
	publisher = {IEEE Computer Society},
	address = {Los Alamitos, CA, USA},
	month = {oct}
}

@article{martins2020sparse,
	title={Sparse and continuous attention mechanisms},
	author={Martins, Andr{\'e} and Farinhas, Ant{\'o}nio and Treviso, Marcos and Niculae, Vlad and Aguiar, Pedro and Figueiredo, Mario},
	journal={Advances in Neural Information Processing Systems},
	volume={33},
	pages={20989--21001},
	year={2020}
}

@inproceedings{kervadec2021roses,
	title={Roses are red, violets are blue... but should vqa expect them to?},
	author={Kervadec, Corentin and Antipov, Grigory and Baccouche, Moez and Wolf, Christian},
	booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
	pages={2776--2785},
	year={2021}
}

@inproceedings{hudson2019gqa,
	title={GQA: A new dataset for real-world visual reasoning and compositional question answering},
	author={Hudson, Drew A and Manning, Christopher D},
	booktitle={Proceedings of the IEEE/CVF conference on computer vision and pattern recognition},
	pages={6700--6709},
	year={2019}
}
@INPROCEEDINGS{teney2020unshuffling,
	author = {D. Teney and E. Abbasnejad and A. van den Hengel},
	booktitle = {2021 IEEE/CVF International Conference on Computer Vision (ICCV)},
	title = {Unshuffling Data for Improved Generalization in Visual Question Answering},
	year = {2021},
	volume = {},
	issn = {},
	pages = {1397-1407},
	doi = {10.1109/ICCV48922.2021.00145},
	url = {https://doi.ieeecomputersociety.org/10.1109/ICCV48922.2021.00145},
	publisher = {IEEE Computer Society},
	address = {Los Alamitos, CA, USA},
	month = {oct}
}
@inproceedings{hudson2018compositional,
	title={Compositional Attention Networks for Machine Reasoning},
	author={Hudson, Drew A and Manning, Christopher D},
	booktitle={International Conference on Learning Representations (ICLR)},
	year={2018}
}
@inproceedings{clark2019dont,
	title = "Don{'}t Take the Easy Way Out: Ensemble Based Methods for Avoiding Known Dataset Biases",
	author = "Clark, Christopher  and
	Yatskar, Mark  and
	Zettlemoyer, Luke",
	booktitle = "Proceedings of the 2019 Conference on Empirical Methods in Natural Language Processing and the 9th International Joint Conference on Natural Language Processing (EMNLP-IJCNLP)",
	month = nov,
	year = "2019",
	address = "Hong Kong, China",
	publisher = "Association for Computational Linguistics",
	url = "https://aclanthology.org/D19-1418",
	doi = "10.18653/v1/D19-1418",
	pages = "4069--4082",
}

@article{gao2021structured,
	title={Structured multimodal attentions for textvqa},
	author={Gao, Chenyu and Zhu, Qi and Wang, Peng and Li, Hui and Liu, Yuliang and Van den Hengel, Anton and Wu, Qi},
	journal={IEEE Transactions on Pattern Analysis and Machine Intelligence},
	year={2021},
	publisher={IEEE}
}
@InProceedings{MSCOCO,
	author="Lin, Tsung-Yi
	and Maire, Michael
	and Belongie, Serge
	and Hays, James
	and Perona, Pietro
	and Ramanan, Deva
	and Doll{\'a}r, Piotr
	and Zitnick, C. Lawrence",
	editor="Fleet, David
	and Pajdla, Tomas
	and Schiele, Bernt
	and Tuytelaars, Tinne",
	title="Microsoft COCO: Common Objects in Context",
	booktitle="Computer Vision -- ECCV 2014",
	year="2014",
	publisher="Springer International Publishing",
	address="Cham",
	pages="740--755",
	isbn="978-3-319-10602-1"
}

@inproceedings{ban-original,
	author = {Kim, Jin-Hwa and Jun, Jaehyun and Zhang, Byoung-Tak},
	booktitle = {Advances in Neural Information Processing Systems},
	editor = {S. Bengio and H. Wallach and H. Larochelle and K. Grauman and N. Cesa-Bianchi and R. Garnett},
	pages = {},
	publisher = {Curran Associates, Inc.},
	title = {Bilinear Attention Networks},
	url = {https://proceedings.neurips.cc/paper_files/paper/2018/file/96ea64f3a1aa2fd00c72faacf0cb8ac9-Paper.pdf},
	volume = {31},
	year = {2018}
}
@inproceedings{hu2020iterative,
	title={Iterative answer prediction with pointer-augmented multimodal transformers for textvqa},
	author={Hu, Ronghang and Singh, Amanpreet and Darrell, Trevor and Rohrbach, Marcus},
	booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
	pages={9992--10002},
	year={2020}
}
@ARTICLE{em-algorithm,
	author={Moon, T.K.},
	journal={IEEE Signal Processing Magazine}, 
	title={The expectation-maximization algorithm}, 
	year={1996},
	volume={13},
	number={6},
	pages={47-60},
	doi={10.1109/79.543975}}
@inproceedings{yang2021tap,
	title={Tap: Text-aware pre-training for text-vqa and text-caption},
	author={Yang, Zhengyuan and Lu, Yijuan and Wang, Jianfeng and Yin, Xi and Florencio, Dinei and Wang, Lijuan and Zhang, Cha and Zhang, Lei and Luo, Jiebo},
	booktitle={Proceedings of the IEEE/CVF conference on computer vision and pattern recognition},
	pages={8751--8761},
	year={2021}
}
@article{bic-algorithm,
	ISSN = {00905364},
	URL = {http://www.jstor.org/stable/2958889},
	author = {Gideon Schwarz},
	journal = {The Annals of Statistics},
	number = {2},
	pages = {461--464},
	publisher = {Institute of Mathematical Statistics},
	title = {Estimating the Dimension of a Model},
	urldate = {2023-03-22},
	volume = {6},
	year = {1978}
}
@article{js-divergence,
	title={The jensen-shannon divergence},
	author={Men{\'e}ndez, ML and Pardo, JA and Pardo, L and Pardo, MC},
	journal={Journal of the Franklin Institute},
	volume={334},
	number={2},
	pages={307--318},
	year={1997},
	publisher={Elsevier}
}
 @misc{mdl-algorithm, title={Stochastic complexity in Statistical Inquiry}, url={https://www.worldscientific.com/worldscibooks/10.1142/0822#t=aboutBook}, journal={World Scientific}, author={Rissanen, J}, year={1998}} 
@inproceedings{mmnas-original,
	author = {Yu, Zhou and Cui, Yuhao and Yu, Jun and Wang, Meng and Tao, Dacheng and Tian, Qi},
	title = {Deep Multimodal Neural Architecture Search},
	year = {2020},
	isbn = {9781450379885},
	publisher = {Association for Computing Machinery},
	address = {New York, NY, USA},
	url = {https://doi.org/10.1145/3394171.3413977},
	doi = {10.1145/3394171.3413977},
	booktitle = {Proceedings of the 28th ACM International Conference on Multimedia},
	pages = {3743–3752},
	numpages = {10},
	keywords = {neural architecture search, neural networks, multimodal learning},
	location = {Seattle, WA, USA},
	series = {MM '20}
}
@inproceedings{NSM_graphhopper,
 author = {Hudson, Drew and Manning, Christopher D},
 booktitle = {Advances in Neural Information Processing Systems},
 editor = {H. Wallach and H. Larochelle and A. Beygelzimer and F. d\textquotesingle Alch\'{e}-Buc and E. Fox and R. Garnett},
 pages = {},
 publisher = {Curran Associates, Inc.},
 title = {Learning by Abstraction: The Neural State Machine},
 url = {https://proceedings.neurips.cc/paper_files/paper/2019/file/c20a7ce2a627ba838cfbff082db35197-Paper.pdf},
 volume = {32},
 year = {2019}
}
@INPROCEEDINGS{mdetr-original,
	author={Kamath, Aishwarya and Singh, Mannat and LeCun, Yann and Synnaeve, Gabriel and Misra, Ishan and Carion, Nicolas},
	booktitle={2021 IEEE/CVF International Conference on Computer Vision (ICCV)}, 
	title={MDETR - Modulated Detection for End-to-End Multi-Modal Understanding}, 
	year={2021},
	volume={},
	number={},
	pages={1760-1770},
	doi={10.1109/ICCV48922.2021.00180}
}

@INPROCEEDINGS{mcan-original,
	author={Yu, Zhou and Yu, Jun and Cui, Yuhao and Tao, Dacheng and Tian, Qi},
	booktitle={2019 IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR)}, 
	title={Deep Modular Co-Attention Networks for Visual Question Answering}, 
	year={2019},
	volume={},
	number={},
	pages={6274-6283},
	doi={10.1109/CVPR.2019.00644}}

@inproceedings{chen2021zero,
	title={Zero-shot visual question answering using knowledge graph},
	author={Chen, Zhuo and Chen, Jiaoyan and Geng, Yuxia and Pan, Jeff Z and Yuan, Zonggang and Chen, Huajun},
	booktitle={International Semantic Web Conference},
	pages={146--162},
	year={2021},
	organization={Springer}
}
@article{wang2016fvqa,
	author = {Wang, Peng and Wu, Qi and Shen, Chunhua and Dick, Anthony and van den Hengel, Anton},
	title = {FVQA: Fact-Based Visual Question Answering},
	year = {2018},
	issue_date = {October 2018},
	publisher = {IEEE Computer Society},
	address = {USA},
	volume = {40},
	number = {10},
	issn = {0162-8828},
	url = {https://doi.org/10.1109/TPAMI.2017.2754246},
	doi = {10.1109/TPAMI.2017.2754246},
	journal = {IEEE Trans. Pattern Anal. Mach. Intell.},
	month = {oct},
	pages = {2413–2427},
	numpages = {15}
}

@inproceedings{zhang2021devlbert,
	title={DeVLBert: Out-of-distribution Visio-Linguistic Pretraining with Causality},
	author={Zhang, Shengyu and Jiang, Tan and Wang, Tan and Kuang, Kun and Zhao, Zhou and Zhu, Jianke and Yu, Jin and Yang, Hongxia and Wu, Fei},
	booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
	pages={1744--1747},
	year={2021}
}
@article{ali2020metricHitAtK,
	author = {Ali, Mehdi and Berrendorf, Max and Hoyt, Charles and Vermue, Laurent and Galkin, Mikhail and Sharifzadeh, Sahand and Fischer, Asja and Tresp, Volker and Lehmann, Jens},
	year = {2021},
	month = {11},
	pages = {1-1},
	title = {Bringing Light Into the Dark: A Large-Scale Evaluation of Knowledge Graph Embedding Models Under a Unified Framework},
	volume = {PP},
	journal = {IEEE Transactions on Pattern Analysis and Machine Intelligence},
	doi = {10.1109/TPAMI.2021.3124805}
}

@inproceedings{zhan2020medvqa,
	author = {Zhan, Li-Ming and Liu, Bo and Fan, Lu and Chen, Jiaxin and Wu, Xiao-Ming},
	title = {Medical Visual Question Answering via Conditional Reasoning},
	year = {2020},
	isbn = {9781450379885},
	publisher = {Association for Computing Machinery},
	address = {New York, NY, USA},
	url = {https://doi.org/10.1145/3394171.3413761},
	doi = {10.1145/3394171.3413761},
	abstract = {Medical visual question answering (Med-VQA) aims to accurately answer a clinical question presented with a medical image. Despite its enormous potential in healthcare industry and services, the technology is still in its infancy and is far from practical use. Med-VQA tasks are highly challenging due to the massive diversity of clinical questions and the disparity of required visual reasoning skills for different types of questions. In this paper, we propose a novel conditional reasoning framework for Med-VQA, aiming to automatically learn effective reasoning skills for various Med-VQA tasks. Particularly, we develop a question-conditioned reasoning module to guide the importance selection over multimodal fusion features. Considering the different nature of closed-ended and open-ended Med-VQA tasks, we further propose a type-conditioned reasoning module to learn a different set of reasoning skills for the two types of tasks separately. Our conditional reasoning framework can be easily applied to existing Med-VQA systems to bring performance gains. In the experiments, we build our system on top of a recent state-of-the-art Med-VQA model and evaluate it on the VQA-RAD benchmark. Remarkably, our system achieves significantly increased accuracy in predicting answers to both closed-ended and open-ended questions, especially for open-ended questions, where a 10.8\% increase in absolute accuracy is obtained. The source code can be downloaded from https://github.com/awenbocc/med-vqa.},
	booktitle = {Proceedings of the 28th ACM International Conference on Multimedia},
	pages = {2345–2354},
	numpages = {10},
	keywords = {conditional reasoning, attention mechanism, medical visual question answering},
	location = {Seattle, WA, USA},
	series = {MM '20}
}
@InProceedings{vatsal2020iqvqa,
	author="Goel, Vatsal
	and Chandak, Mohit
	and Anand, Ashish
	and Guha, Prithwijit",
	editor="Del Bimbo, Alberto
	and Cucchiara, Rita
	and Sclaroff, Stan
	and Farinella, Giovanni Maria
	and Mei, Tao
	and Bertini, Marco
	and Escalante, Hugo Jair
	and Vezzani, Roberto",
	title="IQ-VQA: Intelligent Visual Question Answering",
	booktitle="Pattern Recognition. ICPR International Workshops and Challenges",
	year="2021",
	publisher="Springer International Publishing",
	address="Cham",
	pages="357--370",
	isbn="978-3-030-68790-8"
}
@INPROCEEDINGS{spencer2021skill,
	author = {S. Whitehead and H. Wu and H. Ji and R. Feris and K. Saenko},
	booktitle = {2021 IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR)},
	title = {Separating Skills and Concepts for Novel Visual Question Answering},
	year = {2021},
	volume = {},
	issn = {},
	pages = {5628-5637},
	doi = {10.1109/CVPR46437.2021.00558},
	url = {https://doi.ieeecomputersociety.org/10.1109/CVPR46437.2021.00558},
	publisher = {IEEE Computer Society},
	address = {Los Alamitos, CA, USA},
	month = {jun}
}

@inproceedings{
	wen2021debiased,
	title={Debiased Visual Question Answering from Feature and Sample Perspectives},
	author={Zhiquan Wen and Guanghui Xu and Mingkui Tan and Qingyao Wu and Qi Wu},
	booktitle={Advances in Neural Information Processing Systems},
	editor={A. Beygelzimer and Y. Dauphin and P. Liang and J. Wortman Vaughan},
	year={2021},
	url={https://openreview.net/forum?id=Z4ry59PVMq8}
}

@InProceedings{rajar2021graphhopper,
	author="Koner, Rajat
	and Li, Hang
	and Hildebrandt, Marcel
	and Das, Deepan
	and Tresp, Volker
	and G{\"u}nnemann, Stephan",
	editor="Hotho, Andreas
	and Blomqvist, Eva
	and Dietze, Stefan
	and Fokoue, Achille
	and Ding, Ying
	and Barnaghi, Payam
	and Haller, Armin
	and Dragoni, Mauro
	and Alani, Harith",
	title="Graphhopper: Multi-hop Scene Graph Reasoning for Visual Question Answering",
	booktitle="The Semantic Web -- ISWC 2021",
	year="2021",
	publisher="Springer International Publishing",
	address="Cham",
	pages="111--127",
	isbn="978-3-030-88361-4"
}
@inproceedings{claudio2019psycholinguistics,
	title = "Psycholinguistics Meets Continual Learning: Measuring Catastrophic Forgetting in Visual Question Answering",
	author = "Greco, Claudio  and
	Plank, Barbara  and
	Fern{\'a}ndez, Raquel  and
	Bernardi, Raffaella",
	booktitle = "Proceedings of the 57th Annual Meeting of the Association for Computational Linguistics",
	month = jul,
	year = "2019",
	address = "Florence, Italy",
	publisher = "Association for Computational Linguistics",
	url = "https://aclanthology.org/P19-1350",
	doi = "10.18653/v1/P19-1350",
	pages = "3601--3605"
}
@inproceedings{niu2021counterfactual,
	author    = {Yulei Niu and
	Kaihua Tang and
	Hanwang Zhang and
	Zhiwu Lu and
	Xian{-}Sheng Hua and
	Ji{-}Rong Wen},
	title     = {Counterfactual {VQA:} {A} Cause-Effect Look at Language Bias},
	booktitle = {{IEEE} Conference on Computer Vision and Pattern Recognition, {CVPR}
	2021, virtual, June 19-25, 2021},
	pages     = {12700--12710},
	publisher = {Computer Vision Foundation / {IEEE}},
	year      = {2021},
	url       = {https://openaccess.thecvf.com/content/CVPR2021/html/Niu\_Counterfactual\_VQA\_A\_Cause-Effect\_Look\_at\_Language\_Bias\_CVPR\_2021\_paper.html},
	doi       = {10.1109/CVPR46437.2021.01251},
	timestamp = {Sun, 02 Oct 2022 15:58:35 +0200},
	biburl    = {https://dblp.org/rec/conf/cvpr/NiuTZL0W21.bib},
	bibsource = {dblp computer science bibliography, https://dblp.org}
}
@inproceedings{zhu2020overcoming,
	title     = {Overcoming Language Priors with Self-supervised Learning for Visual Question Answering},
	author    = {Zhu, Xi and Mao, Zhendong and Liu, Chunxiao and Zhang, Peng and Wang, Bin and Zhang, Yongdong},
	booktitle = {Proceedings of the Twenty-Ninth International Joint Conference on
	Artificial Intelligence, {IJCAI-20}},
	publisher = {International Joint Conferences on Artificial Intelligence Organization},             
	editor    = {Christian Bessiere},	
	pages     = {1083--1089},
	year      = {2020},
	month     = {7},
	note      = {Main track},
	doi       = {10.24963/ijcai.2020/151},
	url       = {https://doi.org/10.24963/ijcai.2020/151},
}
@inproceedings{gokhale2020mutant,
	title = "{MUTANT}: A Training Paradigm for Out-of-Distribution Generalization in Visual Question Answering",
	author = "Gokhale, Tejas  and
	Banerjee, Pratyay  and
	Baral, Chitta  and
	Yang, Yezhou",
	booktitle = "Proceedings of the 2020 Conference on Empirical Methods in Natural Language Processing (EMNLP)",
	month = nov,
	year = "2020",
	address = "Online",
	publisher = "Association for Computational Linguistics",
	url = "https://aclanthology.org/2020.emnlp-main.63",
	doi = "10.18653/v1/2020.emnlp-main.63",
	pages = "878--892",
}

@InProceedings{vqacpv2,
	author = {Agrawal, Aishwarya and Batra, Dhruv and Parikh, Devi and Kembhavi, Aniruddha},
	title = {Don't Just Assume; Look and Answer: Overcoming Priors for Visual Question Answering},
	booktitle = {Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition (CVPR)},
	month = {June},
	year = {2018}
}


@inproceedings{radford2021learning,
	title={Learning transferable visual models from natural language supervision},
	author={Radford, Alec and Kim, Jong Wook and Hallacy, Chris and Ramesh, Aditya and Goh, Gabriel and Agarwal, Sandhini and Sastry, Girish and Askell, Amanda and Mishkin, Pamela and Clark, Jack and Krueger, Gretchen and Sutskever, Ilya},
	booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
	pages={1637--1646},
	year={2021}
}

@article{zhang2018attention,
	title={Attention-based deep multiple instance learning for visual concept detection},
	author={Zhang, Chao and Pang, Yanwei and Zhu, Jia and Shi, Cunzhao and Zhang, Jian and Yuan, Chunfeng},
	journal={IEEE Transactions on Multimedia},
	volume={20},
	number={5},
	pages={1152--1165},
	year={2018},
	publisher={IEEE}
}

@inproceedings{jacobs1991adaptive,
	title={Adaptive mixtures of local experts},
	author={Jacobs, Robert A and Jordan, Michael I and Nowlan, Steven J and Hinton, Geoffrey E},
	booktitle={Neural Information Processing Systems},
	pages={895--902},
	year={1991}
}
@INPROCEEDINGS{huang2018densely,
	author={Huang, Gao and Liu, Zhuang and Van Der Maaten, Laurens and Weinberger, Kilian Q.},
	booktitle={2017 IEEE Conference on Computer Vision and Pattern Recognition (CVPR)}, 
	title={Densely Connected Convolutional Networks}, 
	year={2017},
	volume={},
	number={},
	pages={2261-2269},
	doi={10.1109/CVPR.2017.243},
	ISSN={1063-6919},
	month={July},}
@INPROCEEDINGS{kafle2018dvqa,
	author = {K. Kafle and B. Price and S. Cohen and C. Kanan},
	booktitle = {2018 IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR)},
	title = {DVQA: Understanding Data Visualizations via Question Answering},
	year = {2018},
	volume = {},
	issn = {},
	pages = {5648-5656},
	url = {https://doi.ieeecomputersociety.org/10.1109/CVPR.2018.00592},
	publisher = {IEEE Computer Society},
	address = {Los Alamitos, CA, USA},
	month = {jun}
}
@ARTICLE{kahou2018figureqa,
       author = {{Ebrahimi Kahou}, Samira and {Michalski}, Vincent and {Atkinson}, Adam and {Kadar}, Akos and {Trischler}, Adam and {Bengio}, Yoshua},
        title = "{FigureQA: An Annotated Figure Dataset for Visual Reasoning}",
      journal = {arXiv e-prints},
     keywords = {Computer Science - Computer Vision and Pattern Recognition},
         year = 2017,
        month = oct,
          eid = {arXiv:1710.07300},
        pages = {arXiv:1710.07300},
          doi = {10.48550/arXiv.1710.07300},
archivePrefix = {arXiv},
       eprint = {1710.07300},
 primaryClass = {cs.CV},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017arXiv171007300E},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@InProceedings{zhu2016visual7w,
	author = {Zhu, Yuke and Groth, Oliver and Bernstein, Michael and Fei-Fei, Li},
	title = {Visual7W: Grounded Question Answering in Images},
	booktitle = {Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition (CVPR)},
	month = {June},
	year = {2016}
}

@inproceedings{ImageCLEF2021,
	author = {Bogdan Ionescu and Henning Müller and Renaud Péteri and Asma {Ben Abacha} and Mourad Sarrouti and Dina Demner-Fushman and Sadid A. Hasan and Serge Kozlovski and Vitali Liauchuk and Yashin Dicente and Vassili Kovalev and Obioma Pelka and Alba García Seco de Herrera and Janadhip Jacutprakart and Christoph M. Friedrich and Raul Berari and Andrei Tauteanu and Dimitri Fichou and Paul Brie and Mihai Dogariu and Liviu Daniel Ştefan and Mihai Gabriel Constantin and Jon Chamberlain and Antonio Campello and Adrian Clark and Thomas A. Oliver and Hassan Moustahfid and Adrian Popescu and Jérôme Deshayes-Chossart},
	title = {{Overview of the ImageCLEF 2021}: Multimedia Retrieval in Medical, Nature, Internet and Social Media Applications},
	booktitle = {Experimental IR Meets Multilinguality, Multimodality, and Interaction},
	series = {Proceedings of the 12th International Conference of the CLEF Association (CLEF 2021)},
	year = 2021,
	volume = {},
	publisher = {{LNCS} Lecture Notes in Computer Science, Springer},
	pages = {},
	month = {September 21-24},
	address = {Bucharest, Romania}
}

@Inproceedings{ImageCLEFVQA-Med2019,
	author = {Asma {Ben Abacha} and Sadid A. Hasan and Vivek V. Datla and Joey Liu and Dina Demner-Fushman and Henning M\"uller},
	title = {{VQA-Med}: Overview of the Medical Visual Question Answering Task at ImageCLEF 2019},
	booktitle = {CLEF2019 Working Notes},
	series = {{CEUR} Workshop Proceedings},
	year = {2019},
	volume = {},
	publisher = {CEUR-WS.org $<$http://ceur-ws.org$>$},
	pages = {},
	month = {September 09-12},
	address = {Lugano, Switzerland},
}

@Inproceedings{ImageCLEF-VQA-Med2020,
	author = {Asma {Ben Abacha} and Vivek V. Datla and Sadid A. Hasan and Dina Demner-Fushman and Henning M\"uller},
	title = {Overview of the VQA-Med Task at ImageCLEF 2020: Visual Question Answering and Generation in the Medical Domain}, 
	booktitle = {CLEF 2020 Working Notes},
	series = {{CEUR} Workshop Proceedings},
	year = {2020},
	volume = {},
	publisher = {CEUR-WS.org},
	pages = {},
	month = {September 22-25},
	address = {Thessaloniki, Greece}
}

@ARTICLE{6064996,
  author={Bostock, Michael and Ogievetsky, Vadim and Heer, Jeffrey},
  journal={IEEE Transactions on Visualization and Computer Graphics}, 
  title={D³ Data-Driven Documents}, 
  year={2011},
  volume={17},
  number={12},
  pages={2301-2309},
  doi={10.1109/TVCG.2011.185}
}

@inproceedings{NEURIPS2019_bdbca288,
 author = {Paszke, Adam and Gross, Sam and Massa, Francisco and Lerer, Adam and Bradbury, James and Chanan, Gregory and Killeen, Trevor and Lin, Zeming and Gimelshein, Natalia and Antiga, Luca and Desmaison, Alban and Kopf, Andreas and Yang, Edward and DeVito, Zachary and Raison, Martin and Tejani, Alykhan and Chilamkurthy, Sasank and Steiner, Benoit and Fang, Lu and Bai, Junjie and Chintala, Soumith},
 booktitle = {Advances in Neural Information Processing Systems},
 editor = {H. Wallach and H. Larochelle and A. Beygelzimer and F. d\textquotesingle Alch\'{e}-Buc and E. Fox and R. Garnett},
 pages = {},
 publisher = {Curran Associates, Inc.},
 title = {PyTorch: An Imperative Style, High-Performance Deep Learning Library},
 url = {https://proceedings.neurips.cc/paper_files/paper/2019/file/bdbca288fee7f92f2bfa9f7012727740-Paper.pdf},
 volume = {32},
 year = {2019}
}
@article{jaunet2021visqa,
	TITLE = {{VisQA: X-raying Vision and Language Reasoning in Transformers}},
	AUTHOR = {Jaunet, Theo and Kervadec, Corentin and Vuillemot, Romain and Antipov, Grigory and Baccouche, Moez and Wolf, Christian},
	URL = {https://hal.science/hal-03293079},
	JOURNAL = {{IEEE Transactions on Visualization and Computer Graphics}},
	PUBLISHER = {{Institute of Electrical and Electronics Engineers}},
	YEAR = {2021},
	MONTH = Aug,
	DOI = {10.1109/TVCG.2021.3114683},
	KEYWORDS = {Transformers ; Visual Question Answering ; Visual analytics ; XAI},
	PDF = {https://hal.science/hal-03293079/file/_VIS_21__VisQA_Camera_ready.pdf},
	HAL_ID = {hal-03293079},
	HAL_VERSION = {v1},
}

@inproceedings{bottomup,
	author={Anderson, Peter and He, Xiaodong and Buehler, Chris and Teney, Damien and Johnson, Mark and Gould, Stephen and Zhang, Lei},
	booktitle={2018 IEEE/CVF Conference on Computer Vision and Pattern Recognition}, 
	title={Bottom-Up and Top-Down Attention for Image Captioning and Visual Question Answering}, 
	year={2018},
	volume={},
	number={},
	pages={6077-6086},
	doi={10.1109/CVPR.2018.00636}}

@inproceedings{Khan2022WeaklySG,
	title={Weakly Supervised Grounding for VQA in Vision-Language Transformers},
	author={Aisha Urooj Khan and Hilde Kuehne and Chuang Gan and Niels da Vitoria Lobo and Mubarak Shah},
	year={2022}
}

@inproceedings{NIPS2017_3f5ee243,
	author = {Vaswani, Ashish and Shazeer, Noam and Parmar, Niki and Uszkoreit, Jakob and Jones, Llion and Gomez, Aidan N and Kaiser, \L ukasz and Polosukhin, Illia},
	booktitle = {Advances in Neural Information Processing Systems},
	editor = {I. Guyon and U. Von Luxburg and S. Bengio and H. Wallach and R. Fergus and S. Vishwanathan and R. Garnett},
	pages = {},
	publisher = {Curran Associates, Inc.},
	title = {Attention is All you Need},
	url = {https://proceedings.neurips.cc/paper_files/paper/2017/file/3f5ee243547dee91fbd053c1c4a845aa-Paper.pdf},
	volume = {30},
	year = {2017}
}

@inproceedings{he2016residual,
	added-at = {2021-05-01T22:31:00.000+0200},
	author = {He, Kaiming and Zhang, Xiangyu and Ren, Shaoqing and Sun, Jian},
	biburl = {https://www.bibsonomy.org/bibtex/2f08d8f1a1881a5c9ee27060e40ada500/nosebrain},
	booktitle = {Proceedings of 2016 IEEE Conference on Computer Vision and Pattern Recognition},
	doi = {10.1109/CVPR.2016.90},
	interhash = {d2fe72bcc2c02bacc9fae990ec4d4927},
	intrahash = {f08d8f1a1881a5c9ee27060e40ada500},
	issn = {1063-6919},
	keywords = {image recognition resnet},
	location = {Las Vegas, NV, USA},
	month = jun,
	pages = {770--778},
	publisher = {IEEE},
	series = {CVPR '16},
	timestamp = {2021-05-01T22:31:00.000+0200},
	title = {{Deep Residual Learning for Image Recognition}},
	url = {http://ieeexplore.ieee.org/document/7780459},
	year = 2016
}

@inproceedings{NIPS2017_2cad8fa4,
	author = {Sabour, Sara and Frosst, Nicholas and Hinton, Geoffrey E},
	booktitle = {Advances in Neural Information Processing Systems},
	editor = {I. Guyon and U. Von Luxburg and S. Bengio and H. Wallach and R. Fergus and S. Vishwanathan and R. Garnett},
	pages = {},
	publisher = {Curran Associates, Inc.},
	title = {Dynamic Routing Between Capsules},
	url = {https://proceedings.neurips.cc/paper_files/paper/2017/file/2cad8fa47bbef282badbb8de5374b894-Paper.pdf},
	volume = {30},
	year = {2017}
}
@inproceedings{Zou2020,
	doi = {10.1109/itca52113.2020.00069},
	url = {https://doi.org/10.1109\%2Fitca52113.2020.00069},
	year = 2020,
	month = {dec},
	publisher = {{IEEE}},
	author = {Yeyun Zou and Qiyu Xie},
	title = {A Survey on {VQA}: Datasets and Approaches},
	booktitle = {2020 2nd International Conference on Information Technology and Computer Application ({ITCA})}
}

